Aerial Energy Provisioning for Massive Energy-Constrained IoT by UAVs

Autonomy of devices is a major challenge in many Internet of Things (IoT) applications, in particular when the nodes are deployed remotely or difficult to assess places. In this paper we present an approach to provide energy to these devices by Unmanned Aerial Vehicles (UAVs). Therefore, the two major challenges, finding and charging the node are presented. We propose a model to give the energy constrained node an unlimited autonomy by taken the Wireless Power Transfer (WPT) link and battery capacity into account. Selecting the most suitable battery technology allows a reduction in battery capacity and waste. Moreover, an upgrade of existing IoT nodes is feasible with a limited impact on the design and form factor.

==> Images/rate_aut_bat.tex <==
% This file was created with tikzplotlib v0.9.15.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black,
  font=\footnotesize
},
tick label style = {font = \footnotesize},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={\footnotesize C-rate},
xmin=-0.29, xmax=3.89,
xtick style={color=black},
xtick={0.2,1.2,2.2,3.2},
xticklabels={1C,2C,5C,10C},
y grid style={white!69.0196078431373!black},
ylabel={\footnotesize Autonomy [Years]},
ymin=0, ymax=4,
ytick style={color=black}
]
\draw[draw=none,fill=color0,fill opacity=0.9] (axis cs:-0.1,0) rectangle (axis cs:0.1,0.0849315068493151);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0,fill opacity=0.9}
\addlegendentry{50 mAh}

\draw[draw=none,fill=color0,fill opacity=0.9] (axis cs:0.9,0) rectangle (axis cs:1.1,0.0931506849315069);
\draw[draw=none,fill=color0,fill opacity=0.9] (axis cs:1.9,0) rectangle (axis cs:2.1,0.128767123287671);
\draw[draw=none,fill=color0,fill opacity=0.9] (axis cs:2.9,0) rectangle (axis cs:3.1,0.361643835616438);
\draw[draw=none,fill=color1,fill opacity=0.9] (axis cs:0.1,0) rectangle (axis cs:0.3,0.186301369863014);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1,fill opacity=0.9}
\addlegendentry{100 mAh}

\draw[draw=none,fill=color1,fill opacity=0.9] (axis cs:1.1,0) rectangle (axis cs:1.3,0.227397260273973);
\draw[draw=none,fill=color1,fill opacity=0.9] (axis cs:2.1,0) rectangle (axis cs:2.3,0.723287671232877);
\draw[draw=none,fill=color1,fill opacity=0.9] (axis cs:3.1,0) rectangle (axis cs:3.3,5);
\draw[draw=none,fill=color2,fill opacity=0.9] (axis cs:0.3,0) rectangle (axis cs:0.5,0.457534246575342);
\addlegendimage{ybar,ybar legend,draw=none,fill=color2,fill opacity=0.9}
\addlegendentry{200 mAh}

\draw[draw=none,fill=color2,fill opacity=0.9] (axis cs:1.3,0) rectangle (axis cs:1.5,0.838356164383562);
\draw[draw=none,fill=color2,fill opacity=0.9] (axis cs:2.3,0) rectangle (axis cs:2.5,5);
\draw[draw=none,fill=color2,fill opacity=0.9] (axis cs:3.3,0) rectangle (axis cs:3.5,5);
\draw[draw=none,fill=color3,fill opacity=0.9] (axis cs:0.5,0) rectangle (axis cs:0.7,3.61917808219178);
\addlegendimage{ybar,ybar legend,draw=none,fill=color3,fill opacity=0.9}
\addlegendentry{500 mAh}

\draw[draw=none,fill=color3,fill opacity=0.9] (axis cs:1.5,0) rectangle (axis cs:1.7,5);
\draw[draw=none,fill=color3,fill opacity=0.9] (axis cs:2.5,0) rectangle (axis cs:2.7,5);
\draw[draw=none,fill=color3,fill opacity=0.9] (axis cs:3.5,0) rectangle (axis cs:3.7,5);
\end{axis}

\end{tikzpicture}

